Strategic Analysis of Trust Models for User-Centric Networks

We present a strategic analysis of a trust model that has recently been proposed for promoting cooperative behaviour in user-centric networks. The mechanism for cooperation is based on a combination of reputation and virtual currency schemes in which service providers reward paying customers and punish non-paying ones by adjusting their reputation, and hence the price they pay for services. We model and analyse this system using PRISM-games, a tool that performs automated verification and strategy synthesis for stochastic multi-player games using the probabilistic alternating-time temporal logic with rewards (rPATL). We construct optimal strategies for both service users and providers, which expose potential risks of the cooperation mechanism and which we use to devise improvements that counteract these risks.

==> eptcsdata.tex <==
\providecommand{\firstpage}{53}
\providecommand{\publicationstatus}{F. Mogavero, A. Murano, and M.Y. Vardi (Eds.):\\
1st Workshop on Strategic Reasoning 2013 (SR'13)  \\
EPTCS 112, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.112.10}{10.4204/EPTCS.112.10}}
\pdfoutput=1

